Significance Mode Analysis (SigMA) for hierarchical structures. An application to the Sco-Cen OB association

We present a new clustering method, Significance Mode Analysis (SigMA), to extract co-spatial and co-moving stellar populations from large-scale surveys such as ESA Gaia. The method studies the topological properties of the density field in the multidimensional phase space. We validate SigMA on simulated clusters and find that it outperforms competing methods, especially in cases where many clusters are closely spaced. We apply the new method to Gaia DR3 data of the closest OB association to Earth, Scorpio-Centaurus (Sco-Cen), and find more than 13,000 co-moving young objects, with about 19% of these having a sub-stellar mass. SigMA finds 37 co-moving clusters in Sco-Cen. These clusters are independently validated by their narrow HRD sequences and, to a certain extent, by their association with massive stars too bright for Gaia, hence unknown to SigMA. We compare our results with similar recent work and find that the SigMA algorithm recovers richer populations, is able to distinguish clusters with velocity differences down to about 0.5 km s$^{-1}$, and reaches cluster volume densities as low as 0.01 sources/pc$^3$. The 3D distribution of these 37 coeval clusters implies a larger extent and volume for the Sco-Cen OB association than typically assumed in the literature. Additionally, we find the association to be more actively star-forming and dynamically more complex than previously thought. We confirm that the star-forming molecular clouds in the Sco-Cen region, namely, Ophiuchus, L134/L183, Pipe Nebula, Corona Australis, Lupus, and Chamaeleon, are part of the Sco-Cen The application of SigMA to Sco-Cen demonstrates that advanced machine learning tools applied to the superb Gaia data allows to construct an accurate census of the young populations, to quantify their dynamics, and to reconstruct the recent star formation history of the local Milky Way.

==> tables/table1.tex <==
\begin{table*}[!ht] 
\begin{center}
\begin{small}
\caption{Average parameters of the 48 SigMA clusters in ScoCen.}
\renewcommand{\arraystretch}{1.2}
\resizebox{1\textwidth}{!}{%
\begin{tabular}{rlllrrrccccccrrr}
\hline \hline
%
\multicolumn{1}{r}{RAG} &
\multicolumn{1}{l}{Region} &
\multicolumn{1}{l}{Group Name} &
\multicolumn{1}{l}{Brightest star} &
\multicolumn{1}{r}{Nr.} &
\multicolumn{1}{c}{$l$} &
\multicolumn{1}{c}{$b$} &
\multicolumn{1}{c}{$\varpi$} &
\multicolumn{1}{c}{$d$} &
% \multicolumn{1}{c}{$\sigma_l$} &
% \multicolumn{1}{c}{$\sigma_b$} &
% \multicolumn{1}{c}{$\alpha$} &
% \multicolumn{1}{c}{$\delta$} &
% \multicolumn{1}{c}{$\sigma_\alpha$} &
% \multicolumn{1}{c}{$\sigma_\delta$} \\
\multicolumn{1}{c}{$\mu_\alpha^*$} &
\multicolumn{1}{c}{$\mu_\delta$} &
% \multicolumn{1}{c}{$\sigma\_\mu_\alpha^*$} &
% \multicolumn{1}{c}{$\sigma\_\mu_\delta$} &
\multicolumn{1}{c}{$v_\alpha$} &
\multicolumn{1}{c}{$v_\delta$} &
% \multicolumn{1}{c}{$\sigma\_v_\alpha$} &
% \multicolumn{1}{c}{$\sigma\_v_\delta$} \\
\multicolumn{1}{c}{$X$} &
\multicolumn{1}{c}{$Y$} &
\multicolumn{1}{c}{$Z$} \\
%
& & & & &
\multicolumn{2}{c}{(deg)} & 
% \multicolumn{1}{c}{(deg)} &
\multicolumn{1}{c}{(mas)} & 
\multicolumn{1}{c}{(pc)} &
% \multicolumn{1}{c}{(deg)} & 
% \multicolumn{1}{c}{(deg)} &
% \multicolumn{1}{c}{(deg)} & 
% \multicolumn{1}{c}{(deg)} \\
\multicolumn{2}{c}{(mas/yr)} &
% \multicolumn{1}{c}{(mas/yr)} &
% \multicolumn{1}{c}{(mas/yr)} &
% \multicolumn{1}{c}{(mas/yr)} &
\multicolumn{2}{c}{(km/s)} &
% \multicolumn{1}{c}{(km/s)} &
% \multicolumn{1}{c}{(km/s)} &
% \multicolumn{1}{c}{(km/s)} \\
\multicolumn{1}{c}{(pc)} &
\multicolumn{1}{c}{(pc)} &
\multicolumn{1}{c}{(pc)} \\
\hline

1 & Pipe & B59 & AS 220 & 21 & 357.09 & 7.07 & 6.218 & 161 & -0.35 & -18.94 & -0.26 & -14.42 & 159.67 & -8.20 & 19.76 \\
2 & Cham & Chamaeleon-1 & CV Cha & 148 & 297.23 & -15.44 & 5.231 & 191 & -22.54 & 0.30 & -20.32 & 0.27 & 83.99 & -164.35 & -50.00 \\
3 & Cham & Chamaeleon-2 & Hen 3-854 & 40 & 303.68 & -14.71 & 5.085 & 197 & -20.22 & -7.52 & -18.95 & -7.01 & 105.35 & -158.52 & -49.73 \\
4 & US & rho Oph/L1688 & i Sco & 463 & 353.20 & 16.99 & 7.195 & 139 & -6.80 & -25.97 & -4.49 & -16.98 & 131.69 & -15.82 & 40.70 \\
5 & UCL & Lupus-3 & LL Lup & 139 & 339.56 & 9.44 & 6.277 & 159 & -10.13 & -23.48 & -7.56 & -17.86 & 147.34 & -54.68 & 26.20 \\
6 & UCL & Lupus-4 & MY Lup & 23 & 336.09 & 8.35 & 6.245 & 160 & -11.11 & -23.51 & -8.39 & -17.87 & 144.53 & -63.75 & 23.43 \\
7 & US & nu Sco & nu Sco & 139 & 354.56 & 22.89 & 7.181 & 139 & -8.48 & -24.35 & -5.62 & -16.12 & 127.55 & -12.12 & 54.20 \\
8 & US & delta Sco & ome Sco & 388 & 350.65 & 22.08 & 7.049 & 142 & -11.69 & -23.99 & -7.83 & -16.20 & 129.50 & -21.40 & 53.29 \\
9 & US & beta Sco & HD144273 & 147 & 353.40 & 23.84 & 6.540 & 153 & -9.67 & -21.54 & -7.01 & -15.63 & 138.85 & -16.09 & 61.80 \\
10 & US & L183/L134 & HD141569 & 20 & 358.12 & 36.92 & 8.854 & 113 & -17.53 & -20.28 & -9.69 & -10.85 & 90.57 & -3.05 & 67.43 \\
11 & LCC & eta Cham & eta Cha & 20 & 292.46 & -21.64 & 10.137 & 99 & -30.05 & 26.89 & -14.06 & 12.56 & 34.92 & -84.67 & -36.33 \\
12 & LCC & eps Cham & DX Cha & 41 & 300.23 & -15.59 & 9.807 & 102 & -41.03 & -5.76 & -19.79 & -2.81 & 49.64 & -85.09 & -27.52 \\
13 & US & beta Sco-South & HD146367 & 28 & 352.21 & 20.26 & 6.449 & 155 & -8.33 & -23.57 & -6.15 & -17.37 & 144.22 & -19.80 & 53.85 \\
14 & CrA & Corona Australis & HD176270 & 124 & 359.86 & -17.66 & 6.485 & 154 & 4.36 & -27.16 & 3.20 & -19.81 & 147.07 & -0.37 & -46.80 \\
15 & Pipe & Sgr-West & HD163296 & 15 & 7.24 & 1.36 & 9.963 & 100 & -5.95 & -39.55 & -2.80 & -18.93 & 99.17 & 12.71 & 2.43 \\
16 & US & sigma Sco & c02 Sco & 354 & 351.16 & 17.82 & 6.271 & 159 & -10.60 & -21.56 & -8.03 & -16.45 & 149.80 & -23.50 & 48.90 \\
17 & LCC & Musca-foreground & HD104600 & 67 & 300.48 & -10.02 & 9.748 & 103 & -39.37 & -9.40 & -19.20 & -4.50 & 51.54 & -86.34 & -17.73 \\
18 & LCC & Centaurus-Far & HD121808 & 24 & 311.18 & 0.03 & 5.523 & 181 & -19.77 & -14.27 & -17.00 & -12.23 & 118.93 & -137.99 & 0.10 \\
19 & US & Antares & HD146001 & 449 & 352.81 & 17.21 & 7.209 & 139 & -11.16 & -23.68 & -7.35 & -15.62 & 131.14 & -16.51 & 41.24 \\
20 & LCC & alpha Musca & HD112383 & 64 & 302.47 & -5.87 & 9.700 & 103 & -38.10 & -13.67 & -18.63 & -6.69 & 55.41 & -86.51 & -10.54 \\
21 & CrA & CrA-North & HD 172910 & 265 & 359.05 & -13.66 & 6.753 & 148 & 0.84 & -27.67 & 0.58 & -19.43 & 144.02 & -2.41 & -35.12 \\
22 & Pipe & Pipe-foreground & CD-25-12033 & 29 & 0.13 & 8.03 & 9.646 & 104 & -13.37 & -33.67 & -6.49 & -16.66 & 102.62 & 0.23 & 14.30 \\
23 & UCL & epsilon Norma & eps Nor & 69 & 335.65 & 5.02 & 5.512 & 181 & -14.38 & -19.82 & -12.26 & -17.34 & 164.14 & -75.19 & 16.45 \\
24 & LCC & Acrux & zet Cru & 215 & 299.76 & -1.51 & 9.347 & 107 & -37.92 & -10.56 & -19.20 & -5.33 & 52.62 & -92.70 & -2.87 \\
25 & Pipe & Pipe-North & HD155427 & 22 & 4.85 & 12.73 & 7.554 & 132 & -4.93 & -23.36 & -3.11 & -14.60 & 128.37 & 10.87 & 28.91 \\
26 & CrA & Scorpio-Sting & HD159807 & 36 & 350.63 & -5.96 & 6.973 & 143 & -7.65 & -29.54 & -5.20 & -19.82 & 140.06 & -22.72 & -14.71 \\
27 & UCL & V1062-Sco & mu02 Sco & 794 & 343.30 & 4.58 & 5.658 & 177 & -12.01 & -21.23 & -10.08 & -17.83 & 168.52 & -50.84 & 14.15 \\
28 & UCL & Lupus-West & HD125777 & 112 & 319.89 & 13.74 & 5.960 & 168 & -20.16 & -17.01 & -15.98 & -13.68 & 124.16 & -105.68 & 39.97 \\
29 & UCL & Lupus-1 & HD140817 & 110 & 338.78 & 15.76 & 6.728 & 149 & -16.72 & -23.44 & -11.74 & -16.60 & 133.55 & -52.20 & 40.25 \\
30 & US & Scorpio-Body & HD154310 & 315 & 349.15 & 7.21 & 6.997 & 143 & -8.08 & -26.64 & -5.44 & -17.69 & 139.78 & -26.86 & 17.21 \\
31 & UCL & psi02 Lup & psi02 Lup & 229 & 336.01 & 11.44 & 7.833 & 128 & -19.62 & -28.99 & -11.84 & -17.41 & 113.27 & -49.25 & 25.19 \\
32 & UCL & nu Cen & nu Cen & 897 & 315.41 & 17.77 & 7.365 & 136 & -25.00 & -19.89 & -15.99 & -12.88 & 90.51 & -90.76 & 41.40 \\
33 & UCL & rho Lup & rho Lup & 116 & 321.22 & 12.45 & 8.237 & 121 & -25.42 & -24.86 & -14.56 & -14.26 & 91.09 & -73.64 & 26.41 \\
34 & US & US-foreground-3 & HD151012 & 46 & 349.47 & 11.57 & 8.696 & 115 & -17.71 & -32.12 & -9.43 & -17.47 & 110.58 & -19.29 & 22.84 \\
35 & LCC & sig Cen & sig Cen & 1417 & 300.59 & 7.23 & 8.795 & 114 & -33.82 & -12.66 & -18.40 & -7.15 & 57.79 & -96.82 & 14.11 \\
36 & Pipe & tet Oph & HD158704 & 82 & 359.88 & 7.04 & 6.768 & 148 & -4.71 & -21.70 & -3.28 & -15.37 & 146.72 & -0.32 & 18.49 \\
37 & LCC & f Cen & f Cen & 326 & 306.63 & 12.69 & 8.258 & 121 & -30.71 & -17.18 & -17.62 & -10.03 & 69.67 & -94.86 & 26.35 \\
38 & UCL & V795 Cen & V795 Cen & 351 & 314.28 & 10.11 & 7.652 & 131 & -26.25 & -20.62 & -16.16 & -12.67 & 87.99 & -91.35 & 22.77 \\
39 & UCL & eta Lup & HD 143699 & 242 & 339.42 & 10.92 & 7.244 & 138 & -17.53 & -27.57 & -11.45 & -18.07 & 126.57 & -47.55 & 26.16 \\
40 & UCL & b Cen & b Cen & 546 & 332.51 & 19.59 & 8.133 & 123 & -24.00 & -26.35 & -13.98 & -15.39 & 101.98 & -53.45 & 41.88 \\
41 & UCL & V1019 Cen & HD132238 & 188 & 330.89 & 20.76 & 6.406 & 156 & -16.61 & -20.63 & -12.27 & -15.21 & 127.34 & -70.68 & 55.23 \\
42 & UCL & Lupus-East & HD143022 & 87 & 334.34 & 10.44 & 5.875 & 170 & -16.10 & -19.57 & -12.98 & -15.86 & 149.69 & -71.93 & 30.86 \\
43 & UCL & mu Sco & HD150641 & 80 & 346.02 & 3.87 & 6.065 & 165 & -11.74 & -22.46 & -9.22 & -17.53 & 159.68 & -39.90 & 11.16 \\
44 & US & US-foreground-1 & HD145964 & 170 & 349.32 & 20.59 & 9.151 & 109 & -20.53 & -31.72 & -10.54 & -16.59 & 100.72 & -19.45 & 38.26 \\
45 & US & US-foreground-2 & HD140968 & 59 & 348.60 & 23.25 & 8.109 & 123 & -18.83 & -26.67 & -11.15 & -15.40 & 111.25 & -22.55 & 48.17 \\
46 & UCL & e Lup & e Lup & 139 & 327.85 & 12.07 & 6.851 & 146 & -20.57 & -21.89 & -14.34 & -15.17 & 121.38 & -76.19 & 30.70 \\
47 & UCL & phi02 Lup & HD137432 & 116 & 334.99 & 16.98 & 7.028 & 142 & -19.43 & -23.55 & -13.02 & -15.83 & 122.77 & -57.51 & 41.21 \\
48 & UCL & Libra-South & TYC-6762-602-1 & 38 & 338.31 & 27.51 & 6.558 & 152 & -16.33 & -20.81 & -11.60 & -15.33 & 123.84 & -50.13 & 70.33 \\

\hline
\end{tabular}
} % end resize box
\renewcommand{\arraystretch}{1}
\label{tab:averages}
% \tablefoot{
% \tablefoottext{a}{Some footnote a}
% \tablefoottext{b}{Some footnote b}
% }
\end{small}
\end{center}
\end{table*}

==> tables/table1_sorted.tex <==
\begin{table*}[!ht] 
\begin{center}
\begin{small}
\caption{Average parameters of the 37 \texttt{SigMA} clusters in Sco-Cen, assigned to seven subregions. \vspace{-1mm}}
\renewcommand{\arraystretch}{1.2}
\resizebox{1\textwidth}{!}{%
\begin{tabular}{clllrrrccccccccrrr}
\hline \hline
%
\multicolumn{1}{r}{\texttt{SigMA}} &
% \multicolumn{1}{r}{RAG} &
\multicolumn{1}{l}{Region} &
\multicolumn{1}{l}{Group Name} &
\multicolumn{1}{l}{Brightest star} &
\multicolumn{1}{r}{Nr.} &
\multicolumn{1}{c}{$l$} &
\multicolumn{1}{c}{$b$} &
\multicolumn{1}{c}{$\varpi$} &
\multicolumn{1}{c}{$d$} &
% \multicolumn{1}{c}{$\sigma_l$} &
% \multicolumn{1}{c}{$\sigma_b$} &
% \multicolumn{1}{c}{$\alpha$} &
% \multicolumn{1}{c}{$\delta$} &
% \multicolumn{1}{c}{$\sigma_\alpha$} &
% \multicolumn{1}{c}{$\sigma_\delta$} \\
\multicolumn{1}{c}{$\mu_\alpha^*$} &
\multicolumn{1}{c}{$\mu_\delta$} &
% \multicolumn{1}{c}{$\sigma\_\mu_\alpha^*$} &
% \multicolumn{1}{c}{$\sigma\_\mu_\delta$} &
\multicolumn{1}{c}{$v_\alpha$} &
\multicolumn{1}{c}{$v_\delta$} &
% \multicolumn{1}{c}{$\sigma\_v_\alpha$} &
% \multicolumn{1}{c}{$\sigma\_v_\delta$} \\
\multicolumn{1}{c}{$v_{\alpha,\mathrm{LSR}}$} &
\multicolumn{1}{c}{$v_{\delta,\mathrm{LSR}}$} &
\multicolumn{1}{c}{$X$} &
\multicolumn{1}{c}{$Y$} &
\multicolumn{1}{c}{$Z$} \\
%
& & & & &
\multicolumn{2}{c}{(deg)} & 
% \multicolumn{1}{c}{(deg)} &
\multicolumn{1}{c}{(mas)} & 
\multicolumn{1}{c}{(pc)} &
% \multicolumn{1}{c}{(deg)} & 
% \multicolumn{1}{c}{(deg)} &
% \multicolumn{1}{c}{(deg)} & 
% \multicolumn{1}{c}{(deg)} \\
\multicolumn{2}{c}{(mas/yr)} &
% \multicolumn{1}{c}{(mas/yr)} &
% \multicolumn{1}{c}{(mas/yr)} &
% \multicolumn{1}{c}{(mas/yr)} &
\multicolumn{2}{c}{(km/s)} &
\multicolumn{2}{c}{(km/s)} &
% \multicolumn{1}{c}{(km/s)} &
% \multicolumn{1}{c}{(km/s)} &
% \multicolumn{1}{c}{(km/s)} \\
\multicolumn{1}{c}{(pc)} &
\multicolumn{1}{c}{(pc)} &
\multicolumn{1}{c}{(pc)} \\
\hline

% SIGMA & Region & Group_Name & Brightest_Star & nr_sources & l & b & plx & dist & pmra & pmdec & va & vd & va_lsr & vd_lsr & X & Y & Z \\
1 & US & rho Oph/L1688 & rho Oph & 535 & 353.20 & 17.09 & 7.195 & 139 & -6.81 & -25.91 & -4.50 & -16.95 & 1.36 & -4.20 & 131.88 & -15.88 & 40.87 \\
2 & US & nu Sco & nu Sco & 150 & 354.46 & 22.86 & 7.176 & 139 & -8.47 & -24.50 & -5.61 & -16.22 & 1.21 & -4.52 & 127.69 & -12.31 & 54.45 \\
3 & US & delta Sco & b Sco & 691 & 350.25 & 22.18 & 7.029 & 142 & -12.24 & -23.92 & -8.22 & -16.27 & -0.77 & -3.88 & 129.92 & -22.79 & 53.30 \\
4 & US & beta Sco & HD142883 & 285 & 353.21 & 23.53 & 6.491 & 154 & -9.39 & -21.69 & -6.87 & -15.86 & 0.26 & -4.13 & 140.35 & -16.17 & 61.41 \\
5 & US & sigma Sco & * c02 Sco & 544 & 351.13 & 17.87 & 6.290 & 159 & -10.68 & -21.79 & -8.12 & -16.49 & -1.68 & -3.48 & 149.61 & -23.15 & 48.52 \\
6 & US & Antares & HD146001 & 502 & 352.79 & 17.22 & 7.209 & 139 & -11.00 & -23.31 & -7.23 & -15.52 & -1.29 & -2.43 & 131.34 & -16.59 & 41.42 \\
7 & US & rho Sco & rho Sco & 240 & 349.31 & 18.29 & 7.206 & 139 & -15.98 & -24.14 & -10.44 & -15.82 & -3.64 & -2.78 & 129.71 & -24.38 & 42.91 \\
8 & US & Scorpio-Body & HD150638 & 373 & 349.36 & 7.31 & 7.083 & 141 & -8.04 & -26.82 & -5.30 & -17.64 & -1.38 & -2.83 & 138.01 & -24.51 & 16.90 \\
9 & US & US-foreground & HD145964 & 276 & 348.81 & 21.04 & 9.052 & 110 & -19.97 & -31.25 & -10.63 & -16.28 & -3.33 & -3.86 & 101.01 & -19.28 & 40.39 \\
\hline
10 & UCL & V1062-Sco & mu02 Sco & 1029 & 343.11 & 4.69 & 5.660 & 177 & -12.14 & -21.15 & -10.18 & -17.73 & -5.12 & -2.15 & 168.42 & -51.40 & 14.38 \\
11 & UCL & mu Sco & HD151726 & 54 & 346.19 & 3.90 & 6.065 & 165 & -11.75 & -22.61 & -9.22 & -17.61 & -5.28 & -2.11 & 159.76 & -39.25 & 11.05 \\
12 & UCL & Libra-South & HD138343 & 71 & 341.77 & 27.80 & 6.344 & 158 & -14.87 & -20.92 & -11.15 & -15.44 & -1.00 & -3.71 & 132.57 & -45.44 & 72.14 \\
13 & UCL & Lupus-1-4 & LL Lup & 226 & 339.51 & 9.44 & 6.270 & 160 & -10.54 & -23.39 & -8.07 & -17.77 & -0.76 & -2.85 & 147.24 & -55.30 & 26.51 \\
14 & UCL & eta Lup & eta Lup & 769 & 339.83 & 10.71 & 7.370 & 136 & -17.63 & -27.84 & -11.21 & -17.83 & -4.15 & -3.18 & 125.63 & -44.42 & 25.62 \\
15 & UCL & phi Lup & phi02 Lup & 1114 & 334.17 & 17.69 & 7.654 & 131 & -20.99 & -25.60 & -13.31 & -15.82 & -3.37 & -2.45 & 112.29 & -53.81 & 39.59 \\
16 & UCL & Norma-North & HD143215 & 42 & 331.12 & 6.40 & 9.440 & 106 & -27.93 & -42.80 & -14.07 & -21.39 & -5.73 & -6.05 & 93.50 & -48.95 & 9.18 \\
17 & UCL & e Lup & e Lup & 516 & 327.40 & 11.48 & 6.893 & 145 & -20.80 & -21.67 & -14.44 & -15.07 & -3.81 & -1.05 & 119.53 & -76.69 & 29.60 \\
18 & UCL & UPK606 & HD125777 & 131 & 320.00 & 13.72 & 5.925 & 169 & -20.07 & -17.01 & -15.96 & -13.69 & -3.20 & -1.14 & 125.51 & -105.77 & 39.35 \\
19 & UCL & rho Lup & rho Lup & 246 & 315.12 & 9.83 & 8.162 & 123 & -26.22 & -23.13 & -15.51 & -13.14 & -1.95 & -1.18 & 85.83 & -84.83 & 21.16 \\
20 & UCL & nu Cen & nu Cen & 1737 & 318.50 & 17.45 & 7.208 & 139 & -23.33 & -20.27 & -15.28 & -13.53 & -1.78 & -1.71 & 98.79 & -87.81 & 42.14 \\
\hline
21 & LCC & Centaurus-Far & HD121808 & 99 & 310.69 & -1.18 & 5.252 & 190 & -18.40 & -11.75 & -16.64 & -10.51 & -2.79 & 0.31 & 124.67 & -143.92 & -2.11 \\
22 & LCC & sig Cen & sig Cen & 1805 & 301.56 & 8.35 & 8.708 & 115 & -33.23 & -13.67 & -18.27 & -7.70 & -2.20 & -0.41 & 59.34 & -96.76 & 17.43 \\
23 & LCC & Acrux & zet Crux & 394 & 300.28 & -1.98 & 9.408 & 106 & -37.73 & -11.36 & -19.10 & -5.69 & -2.75 & -0.17 & 53.64 & -91.70 & -3.54 \\
24 & LCC & Musca-foreground & HD107947 & 95 & 300.64 & -10.27 & 9.788 & 102 & -39.37 & -9.33 & -19.20 & -4.49 & -2.84 & -0.23 & 51.24 & -86.52 & -18.06 \\
25 & LCC & eps Cham & DX Cha & 39 & 300.34 & -15.97 & 9.807 & 102 & -41.23 & -6.05 & -19.85 & -2.92 & -3.31 & -0.54 & 49.58 & -84.51 & -28.23 \\
26 & LCC & eta Cham & eta Cha & 30 & 292.49 & -21.60 & 10.145 & 99 & -30.16 & 26.86 & -14.06 & 12.55 & -2.58 & 2.09 & 35.01 & -84.72 & -36.25 \\
\hline
27 & Pipe & B59 & Em* AS 218 & 32 & 357.10 & 7.11 & 6.233 & 160 & -0.49 & -18.84 & -0.37 & -14.48 & 2.14 & -0.61 & 158.98 & -8.12 & 19.89 \\
28 & Pipe & Pipe-North & HD155427 & 42 & 4.92 & 12.85 & 7.691 & 130 & -4.78 & -23.36 & -3.08 & -14.55 & -0.27 & -2.79 & 126.29 & 11.08 & 28.89 \\
29 & Pipe & tet Oph & HD158704 & 98 & 359.71 & 7.05 & 6.788 & 147 & -4.71 & -21.85 & -3.29 & -15.41 & -1.16 & -2.03 & 146.14 & -0.25 & 18.56 \\
\hline
30 & CrA & Corona Australis & HD177076 & 96 & 359.87 & -17.65 & 6.456 & 155 & 4.56 & -27.11 & 3.33 & -19.83 & -1.77 & -4.77 & 147.57 & -0.30 & -47.10 \\
31 & CrA & CrA-North & HD172910 & 351 & 359.02 & -13.98 & 6.702 & 149 & 0.92 & -27.60 & 0.65 & -19.51 & -3.16 & -4.25 & 144.70 & -2.91 & -36.31 \\
32 & CrA & Scorpio-Sting & HD157864 & 132 & 350.59 & -3.04 & 7.488 & 134 & -10.03 & -29.75 & -6.12 & -19.51 & -5.15 & -3.70 & 131.24 & -23.28 & -8.33 \\
\hline
33 & Cham & Chamaeleon-1 & V* CR Cha & 192 & 297.22 & -15.52 & 5.248 & 191 & -22.55 & 0.38 & -20.31 & 0.35 & -3.96 & -0.79 & 83.96 & -163.34 & -50.83 \\
34 & Cham & Chamaeleon-2 & V* BF Cha & 54 & 303.69 & -14.72 & 5.078 & 197 & -20.16 & -7.55 & -18.95 & -7.07 & -3.24 & -0.22 & 105.64 & -158.48 & -50.04 \\
\hline
35 & NE & L134/L183 & HD141569 & 24 & 358.40 & 36.84 & 8.762 & 114 & -17.63 & -20.28 & -9.75 & -11.13 & -0.83 & -2.44 & 91.34 & -1.65 & 68.42 \\
36 & NE & Oph Southeast & HD154922 & 61 & 4.54 & 13.06 & 4.805 & 208 & -5.65 & -11.44 & -5.63 & -11.58 & -2.77 & 0.30 & 202.17 & 16.38 & 46.56 \\
37 & NE & Oph NorthFar & BD-06 4472 & 28 & 9.60 & 24.98 & 5.059 & 198 & -8.57 & -16.75 & -7.78 & -15.89 & -2.83 & -7.11 & 176.47 & 30.69 & 83.58 \\

\hline
\end{tabular}
} % end resize box
\renewcommand{\arraystretch}{1}
\label{tab:averages}
% \tablefoot{
% \tablefoottext{a}{Some footnote a}
% \tablefoottext{b}{Some footnote b}
% }
\end{small}
\end{center}
\end{table*}

==> tables/table2_hip.tex <==
\begin{table*}[!ht] 
\begin{center}
\begin{small}
\caption{Hipparcos astrometry from \citet{VanLeeuwen2007} of bright stellar members in Sco-Cen.}
\renewcommand{\arraystretch}{1.2}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{llclrrcrrr}
\hline \hline
%
\multicolumn{1}{l}{HIP} &
\multicolumn{1}{l}{Name} &
\multicolumn{1}{l}{\texttt{SigMA}\tablefootmark{a}} &
\multicolumn{1}{l}{SpT} &
\multicolumn{1}{c}{$l$} &
\multicolumn{1}{c}{$b$} &
\multicolumn{1}{c}{$\varpi$} &
\multicolumn{1}{c}{$d$\tablefootmark{b}} &
\multicolumn{1}{c}{$\mu_\alpha^*$} &
\multicolumn{1}{c}{$\mu_\delta$} \\
%
& & & &
\multicolumn{2}{c}{(deg)} & 
% \multicolumn{1}{c}{(deg)} &
\multicolumn{1}{c}{(mas)} &
\multicolumn{1}{c}{(pc)} &
\multicolumn{2}{c}{(mas/yr)} \\
% \multicolumn{1}{c}{(mas/yr)} \\
\hline

% HIP & name_star & sigma & SpT & l & b & plx & dist & pmra & pmdec \\
% HIP & name_star & sigma & SpT & l & b & plx & dist & pmra & pmdec \\
80473 & rho Oph & 1 & B2V & 353.69 & 17.69 & 9.03 & 111 & -5.53 & -21.74 \\
80763 & alf Sco (Antares) & 2 & M1Ib + B2.5V & 351.95 & 15.06 & 5.89 & 170 & -12.11 & -23.30 \\
78104 & rho Sco (Iklil) & 3 & B2IV/V & 344.63 & 18.27 & 6.91 & 145 & -15.68 & -24.88 \\
78820 & bet Sco (Acrab) & 4 & B0.5V & 353.19 & 23.60 & 8.07 & 124 & -5.20 & -24.04 \\
80112 & sig Sco (Alniyat) & 5 & B1III & 351.31 & 17.00 & 4.68 & 214 & -10.60 & -16.28 \\
79404 & * c02 Sco & 5 & B2V & 348.12 & 16.84 & 6.81 & 147 & -10.38 & -23.94 \\
78401 & del Sco (Dschubba) & 6 & B0.2IV & 350.10 & 22.49 & 6.64 & 151 & -10.21 & -35.41 \\
79374 & nu Sco (Jabbah) & 7 & B2IV & 354.61 & 22.70 & 6.88 & 145 & -7.65 & -23.71 \\
78533 & V* LL Lup & 10 & Ap Si & 339.64 & 11.41 & 8.61 & 116 & -12.65 & -24.14 \\
81477 & V1062 Sco & 11 & Ap Si & 343.57 & 5.18 & 7.54 & 133 & -10.25 & -21.59 \\
82545 & mu02 Sco (Pipirima) & 11 & B2IV & 346.20 & 3.86 & 6.88 & 145 & -11.09 & -23.32 \\
67464 & nu Cen & 14 & B2IV & 314.41 & 19.89 & 7.47 & 134 & -26.77 & -20.18 \\
71536 & rho Lup & 15 & B5V & 320.13 & 9.86 & 10.32 & 97 & -28.26 & -28.82 \\
78384 & eta Lup & 16 & B2.5IV & 338.77 & 11.01 & 7.38 & 136 & -16.96 & -27.83 \\
82514 & mu01 Sco (Xamidimura) & 17 & B1.5IV + B & 346.12 & 3.91 & 6.51 & 154 & -10.58 & -22.06 \\
75304 & phi02 Lup & 18 & B4V & 333.84 & 16.75 & 6.28 & 159 & -18.24 & -20.72 \\
74449 & e Lup & 19 & B3IV & 327.83 & 11.43 & 6.47 & 155 & -22.01 & -21.75 \\
76371 & d Lup & 19 & B3IVp & 331.02 & 8.76 & 7.62 & 131 & -20.53 & -21.23 \\
42637 & eta Cha & 21 & B9IV & 292.40 & -21.65 & 10.53 & 95 & -28.89 & 27.21 \\
58484 & eps Cha & 22 & B9Vn & 300.21 & -15.62 & 9.02 & 111 & -40.34 & -8.30 \\
60009 & zet Cru & 24 & B2.5V & 299.32 & -1.36 & 9.12 & 110 & -33.80 & -10.15 \\
60718 & alf Cru  (Acrux) & 24 & B0.5IV & 300.13 & -0.36 & 10.13 & 99 & -35.83 & -14.86 \\
60823 & sig Cen & 25 & B3V & 299.10 & 12.47 & 7.92 & 126 & -32.36 & -12.51 \\
84970 & tet Oph & 29 & B2IV & 0.46 & 6.55 & 7.48 & 134 & -7.37 & -23.94 \\

% 80473 & rho Oph & 1 & B2V & 353.69 & 17.69 & 9.03 & 111 & -5.53 & -21.74 \\
% 79374 & nu Sco (Jabbah) & 2 & B2IV & 354.61 & 22.70 & 6.88 & 145 & -7.65 & -23.71 \\
% 78401 & del Sco (Dschubba) & 3 & B0.2IV & 350.10 & 22.49 & 6.64 & 151 & -10.21 & -35.41 \\
% 78820 & bet Sco (Acrab) & 4 & B0.5V & 353.19 & 23.60 & 8.07 & 124 & -5.20 & -24.04 \\
% 80112 & sig Sco (Alniyat) & 6 & B1III & 351.31 & 17.00 & 4.68 & 214 & -10.60 & -16.28 \\
% 80763 & alf Sco (Antares) & 7 & M1Ib+B2.5V & 351.95 & 15.06 & 5.89 & 170 & -12.11 & -23.30 \\
% 80582 & eps Nor & 14 & B4V & 336.00 & 0.98 & 6.15 & 163 & -13.68 & -19.89 \\
% 81477 & V1062 Sco & 15 & ApSi & 343.57 & 5.18 & 7.54 & 133 & -10.25 & -21.59 \\
% 82545 & mu02 Sco & 15 & B2IV & 346.20 & 3.86 & 6.88 & 145 & -11.09 & -23.32 \\
% 76945 & psi02 Lup & 18 & B5V & 338.48 & 16.08 & 8.97 & 111 & -21.37 & -29.98 \\
% 67464 & nu Cen & 19 & B2IV & 314.41 & 19.89 & 7.47 & 134 & -26.77 & -20.18 \\
% 71536 & rho Lup & 20 & B5V & 320.13 & 9.86 & 10.32 & 97 & -28.26 & -28.82 \\
% 69618 & V795 Cen & 21 & B4Vne & 314.13 & 3.96 & 6.77 & 148 & -23.80 & -20.92 \\
% 78384 & eta Lup & 22 & B2.5IV & 338.77 & 11.01 & 7.38 & 136 & -16.96 & -27.83 \\
% 71865 & b Cen & 23 & B2.5V & 325.90 & 20.10 & 9.62 & 104 & -29.92 & -30.68 \\
% 72800 & V1019 Cen & 24 & B7II/III & 327.93 & 19.11 & 6.63 & 151 & -20.48 & -19.20 \\
% 82514 & mu01 Sco & 26 & B1.5IV+B & 346.12 & 3.91 & 6.51 & 154 & -10.58 & -22.06 \\
% 74449 & e Lup & 27 & B3IV & 327.83 & 11.43 & 6.47 & 155 & -22.01 & -21.75 \\
% 75304 & phi02 Lup & 28 & B4V & 333.84 & 16.75 & 6.28 & 159 & -18.24 & -20.72 \\
% 42637 & eta Cha & 30 & B9IV & 292.40 & -21.65 & 10.53 & 95 & -28.89 & 27.21 \\
% 58484 & eps Cha & 31 & B9Vn & 300.21 & -15.62 & 9.02 & 111 & -40.34 & -8.30 \\
% 61585 & alf Mus & 34 & B2IV-V & 301.66 & -6.30 & 10.34 & 97 & -40.20 & -12.80 \\
% 60718 & alf Cru (Acrux) & 35 & B0.5IV & 300.13 & -0.36 & 10.13 & 99 & -35.83 & -14.86 \\
% 60823 & sig Cen & 36 & B3V & 299.10 & 12.47 & 7.92 & 126 & -32.36 & -12.51 \\
% 63945 & f Cen & 37 & B5V & 305.47 & 14.34 & 8.36 & 120 & -29.85 & -15.17 \\
% 84970 & tet Oph & 42 & B2IV & 0.46 & 6.55 & 7.48 & 134 & -7.37 & -23.94 \\

% rho Sco

\hline
\end{tabular}
} % end resizebox
\renewcommand{\arraystretch}{1}
\label{tab:hip}
\tablefoot{Shown are mostly B-type stars that are either part of the \texttt{SigMA} selected clusters, or which are the name-givers of some clusters.
\tablefoottext{a}{Col.~3 gives the index of the \texttt{SigMA} cluster, that is likely related to the given star.}
\tablefoottext{b}{The distance is simply $1000/\varpi$ from Hipparcos, shown here for completeness for an easier comparison with average distances of the \texttt{SigMA} clusters as derived from Gaia parallaxes in Table~\ref{tab:averages}. The Hipparcos distance estimates should be treated with caution, since significant deviations to Gaia distance estimates are possible, while proper motions show deviations on the order of about $\pm2$\,km\,s$^{-1}$ when comparing sources which are both in Hipparcos and Gaia DR3.}
}
\end{small}
\end{center}
\end{table*}

==> tables/table_lit_overview_large.tex <==
\begin{table*}[!ht] 
\begin{center}
\begin{small}
\caption{Overview of the recent Literature to which we compare our results in more detail. @@@We could add such a table, which would make the rough comparisons of total numbers a bit more clear. However, it's really tough to make a nice overview...@@@}
\renewcommand{\arraystretch}{1.2}
\resizebox{1\textwidth}{!}{%
\begin{tabular}{lllllccc}
\hline \hline
\multicolumn{1}{l}{Reference} &
\multicolumn{1}{l}{Data} &
\multicolumn{1}{c}{Studied Area} &
\multicolumn{3}{c}{Number statistics} & %  \tablefootmark{a}
\multicolumn{2}{c}{Only in one or the other} \\
\cmidrule(lr){4-6}
\cmidrule(lr){7-8}
%
\multicolumn{1}{l}{} &
\multicolumn{1}{l}{} &
\multicolumn{1}{c}{} &
\multicolumn{1}{l}{Ref.\tablefootmark{a}} & 
\multicolumn{1}{l}{\texttt{SigMA}\tablefootmark{b}} &
\multicolumn{1}{c}{Matches\tablefootmark{c}} &
\multicolumn{1}{c}{Ref-only} &
\multicolumn{1}{c}{\texttt{SigMA}-only} \\
\hline

% none within 200pc: 3259
% diff within 200pc: 8482
% clus within 200pc: 1703
% both within 200pc: 10185
% all  within 200pc: 13444

% none and seb within 200pc: 198
% diff and seb within 200pc: 5682
% clus and seb within 200pc: 1539
% ic   and seb within 200pc: 0
% both and seb within 200pc: 7221
% all  and seb within 200pc: 7419

\citet{Damiani2019} & Gaia DR2 &  
 $(l = 360^\circ$ to $280^\circ$, $b = 0^\circ$ to $30^\circ)$,
 & 10,185 ($\sim$14\% more)  & 8919 & 7221 & 2964 (We miss 29\%)  & 1698 (\citetalias{Damiani2019} miss 19\%)  \\
 
Sco-Cen &  & $(l = 315^\circ$ to $280^\circ$, $b = -10^\circ$ to $0^\circ)$, & 1703 clustered  &  & 1539 &  110 (We miss 6.5\%) &  \\
 
 & &  FOV = 2750\,deg$^2$, $d<\SI{200}{pc}$ & 8482 diffuse &  & 5682 & 33\% extra diff. & 67\% clust.~in this work \\
\hline



\citet{Kerr2021} & Gaia DR2  & The whole TLC22 stellar group & 7394 & 9598 ($\sim$30\% more) & 5135 & 2259  & 4463  \\
Sco-Cen & & &  &  &  &  &  \\
 \hline

% When comparing the whole TLC22 group (7394) with our Sco-Cen \texttt{SigMA} extraction (without Cham, 9598) we find 5135 cross-matches in total. Hence, 2259 (31\%) sources are only in TLC22, and 4463 are only in \texttt{SigMA}. We find that the \citetalias{Kerr2021} only sample contains older sources when investigating an HRD\footnote{The \citetalias{Kerr2021} PMS selection includes sources up to about 50\,Myr.}, or sources that have deviating motions from \texttt{SigMA} Scon-Cen members, resulting in less than 1/4 of TLC22 only sources that could be young candidate members missed by \texttt{SigMA}.




% 6190 all in Schmitt
% ~1878 30% diffuse
% ~4018 65% clustered in vel-regions where the SigMA clusters fall
% ~294 5% in IC2602 vel-region

% # deZeeuw box:
% lz1,lz2 = 343.,360. # USco
% bz1,bz2 = 10., 30.

% lz3,lz4 = 350.,312. # UCL
% bz3,bz4 = 0., 25.

% lz5,lz6 = 285,312. # LCC
% bz5,bz6 = -10., 22.

% get_dezeeuw = ((l2<=lz2)&(l2>=lz1)&(b<=bz2)&(b>=bz1)) | ((l2<=lz3)&(l2>=lz4)&(b<=bz4)&(b>=bz3)) | ((l2<=lz6)&(l2>=lz5)&(b>=bz5)&(b<=bz6))

% US: $(l = 343^\circ$ to $360^\circ$, $b = 10^\circ$ to $30^\circ) \,\lor$
% UCL: $(l = 312^\circ$ to $350^\circ$, $b = 0^\circ$ to $25^\circ) \,\lor$
% LCC: $(l = 285^\circ$ to $312^\circ$, $b = -10^\circ$ to $22^\circ)$

\citet{Schmitt2022} & Gaia EDR3 \& & \citet{deZeeuw1999} borders: & 6190 & 8593 ($\sim$39\% more) & 2614 & 3576 & 5979 \\
Sco-Cen  & eROSITA & US $(l = 343^\circ$ to $360^\circ$, $b = 10^\circ$ to $30^\circ) \,\lor$  & $\sim$65\% clustered &  & 2614 &  & \\
  &   & UCL $(l = 312^\circ$ to $350^\circ$, $b = 0^\circ$ to $25^\circ) \,\lor$  & $\sim$30\% diffuse &  & 0 &  &  \\
  &  &  LCC $(l = 285^\circ$ to $312^\circ$, $b = -10^\circ$ to $22^\circ)$, & $\sim$5\% IC\,2602 &  & 0 &  &  \\
  &  &  FOV = 2050\,deg$^2$, $d \sim 60$--$\SI{200}{pc}$  &  &  &  &  &  \\
\hline





%  FOV: $l = 2^\circ$ to $283^\circ$ and $b = -12^\circ$ to $35^\circ$} of 3252\,deg$^2$ 
% parallax range: 4-11 mas

% Cross-matching \citetalias{Luhman2022a} with the \texttt{SigMA} clusters gives a total of 7713 matches, 2796  \citetalias{Luhman2022a} only sources, and 1442  \texttt{SigMA} only sources within the \citetalias{Luhman2022a} FOV, where the \texttt{SigMA} sample contains 9155 sources in total.
% %\footnote{Within the \citetalias{Luhman2022a} FOV our sample contains 9155 sources in total.}. 
% % This FOV is slightly smaller than in our work and does not include the southern most parts of Sco-Cen.
% When investigating the 2796 \citetalias{Luhman2022a} only sources, we find that they do not show significant signs of being older than 20\,Myr, or of having significant deviating motions from \texttt{SigMA} Sco-Cen velocities. These extra sources, or part of them, could be Sco-Cen members, meaning we might be missing up to about 1/4 of the candidates. This is not surprising because supervised methods will naturally find more candidates as discussed in Sect.~\ref{sec:damiani}. 

\citet{Luhman2022a} & Gaia EDR3 & $l = 2^\circ$ to $283^\circ$, $b = -12^\circ$ to $35^\circ$, & 10509 & 9155 & 7713  & 2796 & 1442 \\
Sco-Cen  &  & FOV = 3252\,deg$^2$, $d \sim 90$--$\SI{250}{pc}$ &  &  &  &  &  \\
\hline


 
 
 

%   $\alpha = 236^\circ$ to $251^\circ$, $\delta = -29^\circ$ to $-16^\circ$,
% a $20^\circ$ radius around $\alpha$, $\delta$ = $245^\circ$, $-25^\circ$; 
% $d \sim 125$ to 175\,pc.},
% (1442 stars), and into an older diffuse population (1303)
% 2745 total discussed in Squ.

% 1857
% 1199
% 658

\citet{Squicciarini2021} & Gaia EDR3 & $\alpha = 236^\circ$ to $251^\circ$, $\delta = -29^\circ$ to $-16^\circ$ & 2745  & 1918 & 1857 & 888 & 61 \\
Upper-Sco & (subsample with RVs) & FOV = 195\,deg$^2$, $d \sim 125$--$\SI{175}{pc}$ & 1442 clustered &  & 1199 & 243 extra clust.  &  \\
  &  &  & 1303 diffuse &  & 658  & $\sim$50\% extra diff. & $\sim$50\% clust.~in this work \\
 \hline
 
 
 
 
%  2190
% 1623
% 567

% 1680
% 1674
% 1345
% 329

Miret-Roig et al.~(in prep.) & Gaia EDR3 & $\alpha = 235^\circ$ to $252^\circ$, $b = -30^\circ$ to $-16.9^\circ$, & 2190 & 2186 & 1674 & 516 & 512 \\
Upper-Sco & (subsample with RVs) & FOV = 223\,deg$^2$, $d \sim 80$--$\SI{192}{pc}$  & 1623 clustered & -  & 1345 & 278 extra clust. & - \\
 &  & & 567 diffuse & -  & 329 & 238, 42\% extra diff. & $\sim$58\% clust.~in this work \\
 \hline



\hline
\end{tabular}
} % end resizebox
\renewcommand{\arraystretch}{1}
\label{tab:literature}
\tablefoot{
\tablefoottext{a}{Number of stellar members from the given reference. If there was a distinction in the literature between members in a more clustered or diffuse mode, then the numbers are given below.}
\tablefoottext{b}{Number of stellar cluster members from  \texttt{SigMA} in the given studied area (volume), out of the total 9810 \texttt{SigMA} stellar cluster members.}
\tablefoottext{c}{Number of matches between the given reference with \texttt{SigMA} clusters in the given FOV.}
}
\end{small}
\end{center}
\end{table*}

==> tables/table_results_dense.tex <==
\begin{table}[!t] 
\begin{center}
\begin{small}
\caption{Test results on the synthetic ``compact cluster sample''.} % Comparison of \texttt{SigMA} against four other, commonly used density based clustering methods for identifying co-moving groups.}
\renewcommand{\arraystretch}{1.1}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{lllllllll}
\hline \hline\\[-3mm]
\multicolumn{1}{l}{} &
\multicolumn{1}{l}{NMI} &
\multicolumn{1}{l}{AMI} &
\multicolumn{1}{l}{ARI} &
\multicolumn{1}{l}{Recall} &
\multicolumn{1}{l}{Precision} &
\multicolumn{1}{l}{ACC} &
\multicolumn{1}{l}{BACC} & 
\multicolumn{1}{l}{N}
\\[1mm]
\hline\\[-3mm]
\texttt{SigMA} &  &  &  &  &  &  & \\[1mm]
\\[-3mm]
DBSCAN &  &  &  &  &  &  &  \\[1mm]
\\[-3mm]
HDBSCAN &  &  &  &  &  &  &  \\[1mm]
\\[-3mm]
UPMASK &  &  &  &  &  &  &  \\[1mm]
% \\[-3mm]
% EnLink &  &  &  &  &  &  &  \\[1mm]
\hline
\end{tabular}
} % end resize box
\renewcommand{\arraystretch}{1}
\label{tab:results_simulation_dense}
% \tablefoot{
% \tablefoottext{a}{Number of sources from this work, for a direct comparison with the cross-matches as given in brackets in Cols.~4--5.}
% \tablefoottext{b}{The \citetalias{Damiani2019} group shortcuts are given for eight compact clusterings (UCL-1, UCL-2, UCL-3, Lupus 3, LCC-1, US-far, US-near), for four diffuse populations  (D1, D2a, D2b, US-D2), and for sources that have not been assigned to any of these groups (N), while the number in brackets gives the cross-matches with the respective \texttt{SigMA} cluster.}
% \tablefoottext{c}{The \citetalias{Squicciarini2021} groups (G) are numbered from 1 to 8, and their diffuse population is given with D. Again, the number of cross-matches is given in brackets. The eight groups in  \citetalias{Squicciarini2021} are associated with the brightest star in each group as follows: G1--$i$\,Sco; G2--$\nu$\,Sco\,B; G3--$b$\,Sco; G4--HD\,144273; G5--HIP\,77900; G6--HIP\,78968; G7--HIP\,79910; G8--HD\,146467.}
% }
\end{small}
\end{center}
\end{table}


==> tables/table_results_oc.tex <==
\begin{table}[!ht] 
\begin{center}
\begin{small}
\caption{Test results on simulated open cluster sample.} % Comparison of \texttt{SigMA} against four other, commonly used density based clustering methods for identifying co-moving groups.}
\renewcommand{\arraystretch}{1.1}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{lllllllll}
\hline \hline\\[-3mm]
\multicolumn{1}{l}{} &
\multicolumn{1}{l}{NMI} &
\multicolumn{1}{l}{AMI} &
\multicolumn{1}{l}{ARI} &
\multicolumn{1}{l}{Recall} &
\multicolumn{1}{l}{Precision} &
\multicolumn{1}{l}{ACC} &
\multicolumn{1}{l}{BACC} & 
\multicolumn{1}{l}{N}
\\[1mm]
\hline\\[-3mm]
\texttt{SigMA} &  &  &  &  &  &  & \\[1mm]
\\[-3mm]
DBSCAN &  &  &  &  &  &  &  \\[1mm]
\\[-3mm]
HDBSCAN &  &  &  &  &  &  &  \\[1mm]
\\[-3mm]
UPMASK &  &  &  &  &  &  &  \\[1mm]
%\\[-3mm]
%EnLink &  &  &  &  &  &  &  \\[1mm]
\hline
\end{tabular}
} % end resize box
\renewcommand{\arraystretch}{1}
\label{tab:results_simulation_oc}
% \tablefoot{
% \tablefoottext{a}{Number of sources from this work, for a direct comparison with the cross-matches as given in brackets in Cols.~4--5.}
% \tablefoottext{b}{The \citetalias{Damiani2019} group shortcuts are given for eight compact clusterings (UCL-1, UCL-2, UCL-3, Lupus 3, LCC-1, US-far, US-near), for four diffuse populations  (D1, D2a, D2b, US-D2), and for sources that have not been assigned to any of these groups (N), while the number in brackets gives the cross-matches with the respective \texttt{SigMA} cluster.}
% \tablefoottext{c}{The \citetalias{Squicciarini2021} groups (G) are numbered from 1 to 8, and their diffuse population is given with D. Again, the number of cross-matches is given in brackets. The eight groups in  \citetalias{Squicciarini2021} are associated with the brightest star in each group as follows: G1--$i$\,Sco; G2--$\nu$\,Sco\,B; G3--$b$\,Sco; G4--HD\,144273; G5--HIP\,77900; G6--HIP\,78968; G7--HIP\,79910; G8--HD\,146467.}
% }
\end{small}
\end{center}
\end{table}


==> tables/table_results_oc_and_dense.tex <==
\begin{table*}[!ht] 
\begin{center}
\begin{small}
\caption{Test results on simulated cluster samples. Bold faced numbers indicate the best performance given a specific evaluation metric\vspace{-2mm}} % Comparison of \texttt{SigMA} against four other, commonly used density based clustering methods for identifying co-moving groups.}
\renewcommand{\arraystretch}{1.4}
\resizebox{0.99\textwidth}{!}{%
\begin{tabular}{lcccccccccc}
\hline \hline
\multicolumn{1}{l}{} &
\multicolumn{1}{c}{NMI} &
\multicolumn{1}{c}{AMI} &
\multicolumn{1}{c}{ARI} &
\multicolumn{1}{c}{Recall} &
\multicolumn{1}{c}{Precision} &
\multicolumn{1}{c}{ACC} &
\multicolumn{1}{c}{BACC} & 
\multicolumn{1}{c}{MC} & 
\multicolumn{1}{c}{N$_\mathrm{tot}$} &
\multicolumn{1}{c}{N$_\mathrm{cluster}$} \\ 
\hline 
\multicolumn{11}{c}{open cluster sample} \\
\hline
%  Algo & NMI  &  AMI &  ARI &  Rec &  Pre &  ACC & BACC & MC & N_t % N_c \\
\texttt{SigMA} & \textbf{0.95} & \textbf{0.95} & \textbf{0.96} & \textbf{0.97}  & 0.97 & \textbf{0.97} & \textbf{0.90} & \textbf{0.96} & \textbf{12} & \textbf{12} \\ 
DBSCAN  & 0.94 & 0.94 & 0.95 & 0.96 & \textbf{0.98} & 0.96 & 0.88 & 0.95 & \textbf{12} & \textbf{12} \\
HDBSCAN & 0.86 & 0.86 & 0.74 & 0.76 & 0.74 & 0.76 & 0.88 & 0.76 & 14 & \textbf{12} \\ 
%EnLink &  &  &  &  &  &  &  \\ 
\hline
\multicolumn{11}{c}{compact cluster sample} \\
\hline
\texttt{SigMA} & \textbf{0.60} $\pm 0.02$ & \textbf{0.56} $\pm 0.01$ & \textbf{0.38} $\pm 0.03$ & \textbf{0.47} $\pm 0.04$ & \textbf{0.64} $\pm 0.05$ & \textbf{0.47} $\pm 0.04$ &  \textbf{0.51} $\pm 0.04$ & \textbf{0.55} $\pm 0.04$ &  \textbf{26.8} $\pm 2.0$  & \textbf{24.1} $\pm 1.7 $ \\ 
DBSCAN & $0.39 \pm 0.06$ & $0.38 \pm 0.06$ & $0.11 \pm 0.03$ & $0.25 \pm 0.03$ & $0.23 \pm 0.05$ & $0.25 \pm 0.03$ & $0.16 \pm 0.03$ & $0.23 \pm 0.04$ & $10.0 \pm 1.7$ & $10.0 \pm 1.7$ \\ 
HDBSCAN & $0.33 \pm 0.16$ & $0.32 \pm 0.16$ & $0.08 \pm 0.06$ & $0.20 \pm 0.06$ & $0.22 \pm 0.15$ & $0.20 \pm 0.06$ & $0.18 \pm 0.07$ & $0.16 \pm 0.11$ & $24.2 \pm 4.8$ & $12.0 \pm 5.5$ \\
%EnLink &  &  &  &  &  &  &  \\

% 24.2 4.791659420284375
% 12.0 5.477225575051661


% nmi: 0.60 +/- 0.02
% adjusted_mutual_info_score: 0.56 +/- 0.01
% adjusted_rand_score: 0.38 +/- 0.03
% recall: 0.47 +/- 0.04
% precision: 0.64 +/- 0.05
% acc: 0.47 +/- 0.04
% balanced_acc: 0.47 +/- 0.03
% matthews_coef: 0.45 +/- 0.04





\hline
\end{tabular}
} % end resize box
\renewcommand{\arraystretch}{1}
% \label{tab:results_simulation_oc_and_dense}
% \tablefoot{
% \tablefoottext{a}{}
% }
\end{small}
\end{center}
\end{table*}

